Modularity, 4d mirror symmetry, and VOA modules of 4d $\mathcal{N} = 2$ SCFTs with $a = c$

The infinite series of 4d $\mathcal{N} = 2$ SCFTs with central charge relation $a_\text{4d} = c_\text{4d}$ are closely related to the $\mathcal{N}=4$ super Yang-Mills. In this paper we study the modular properties of their associated VOAs $\mathbb{V}[\mathcal{T}_{p,N}]$ where $\mathcal{T}_{p, N}$ are those $a = c$ theories with $SU(N)$ gauge group. We exploit the closed-form formula for the Schur index of the $\mathcal{N} = 4$ $SU(N)$ theories $\mathcal{T}_{SU(N)}$ to derive the space of characters of the VOA $\mathbb{V}[\mathcal{T}_{p,N}]$ and the $S, T$-matrices, and find the (non-monic) modular linear differential equations that constrain the module characters when possible. We investigate the geometric interpretation of some of these modular data through the view point of 4d mirror symmetry. Using insights from the flavored modular differential equation and defect index, we investigate a map between modules characters of $\mathbb{V}[\mathcal{T}_{SU(N)}]$ and those of $\mathbb{V}[\mathcal{T}_{p,N}]$.

==> sections/modular-transformation.tex <==
%!TEX root = ../Schur index and modularity.tex
\subsection{Modular transformation}


